A Modern Search for Wolf-Rayet Stars in the Magellanic Clouds. IV. A Final Census

We summarize the results of our four year survey searching for Wolf-Rayet (WR) stars in the Large Magellanic Cloud (LMC) and Small Magellanic Cloud (SMC). Over the course of this survey we've discovered 15 new WRs and 12 Of-type stars. In this last year we discovered two rare Of-type stars: an O6.5f?p and an O6nfp in addition to the two new Of?p stars discovered in our first year and the three Onfp stars discovered in our second and third years. However, even more exciting was our discovery of a new type of WR, ones we are calling WN3/O3s due to their spectroscopic signatures. We describe the completeness limits of our survey and demonstrate that we are sensitive to weak-lined WRs several magnitudes fainter than any we have discovered, arguing that there is not a population of fainter WRs waiting to be discovered. We discuss the nature of the WN3/O3s, summarizing the results of our extensive spectroscopy and modeling. We also examine the important claim made by others that the WN3/O3s are isolated compared to other massive stars. We find that if we use a more complete sample of reference massive stars, the WN3/O3s show the same spatial distribution as other early WNs, consistent with a common origin. Finally, we use this opportunity to present the "Fifth Catalog of LMC Wolf-Rayet Stars," which includes revised coordinates and updated spectral types for all 154 known LMC WRs.

==> WRCat.tex <==
\begin{deluxetable}{l l l l l l l c l}                                                                                                                
\rotate                                                                                                                                               
\tabletypesize{\scriptsize}                                                                                                                           
\tablecaption{\label{tab:Catalog}The Fifth Catalog of LMC Wolf-Rayet Stars}                                                                               
\tablewidth{0pt}                                                                                                                          
\tablehead{                                                                                                                                           
\colhead{Num.}                                                                                                                                        
& \colhead{$\alpha_{\rm 2000}$}                                                                                                                       
& \colhead{$\delta_{\rm 2000}$}                                                                                                                       
& \colhead{Preferred Name(s)}                                                                                                                                   
& \colhead{$V$}                                                                                                                                       
& \colhead{Type}                                                                                                                                      
& \colhead{Ref.}                                                                                                                                      
& \colhead{OB assoc.\tablenotemark{a}}                                                                                                                
& \colhead{Comments}                                                                                                                                  
}                                                                                                                                                     
\startdata                                                                                                                                            
  1&04 45 32.25  &-70 15 10.9 &BAT99 1;         Brey 1                         &15.78&WN3             &   1,2,3   &\nodata& Runaway?\tablenotemark{b}                         \\     
  2&04 49 36.25  &-69 20 54.8 &BAT99 2;         Brey 2                         &16.58&WN2             &   2       & (1)  &  N\,{\sc v} present but weak; Runaway?\tablenotemark{b}     \\     
  3&04 52 57.39  &-66 41 13.5 &BAT99 3;         Brey 3                         &14.64&WN3             &   1,2,3   &\nodata&                          \\     
  4&04 53 03.76  &-69 23 51.8 &[M2002]LMC 15666                                &14.39&WN3+O6V         &   4       & (2)  & NErn of 2\arcsec pair    \\     
  5&04 53 30.08  &-69 17 49.4 &BAT99 4;         Brey 3a                        &14.27&WNL/Of?        &   5       & (5)  & E. mem.\ of pair.\ Strong neb.\ WR nature unclear\\     
  6&04 54 28.10  &-69 12 50.9 &BAT99 5;         Brey 4                         &16.74&WN2             &   2,3     &    5  & N\,{\sc v} present but weak.     \\     
  7&04 55 07.60  &-69 12 31.7 &BAT99 5a;        [M2002]LMC  23417              &15.30&WN3             &   7       & (5)  &                          \\     
  8&04 55 31.35  &-67 30 02.7 &BAT99 7;         HD 32109                       &13.85&WN3pec          &   3       &\nodata& Lines unusually broad.   \\     
  9&04 56 02.88  &-69 27 21.5 &BAT99 8;         Brey 8;    HD 32257            &14.23&WC4             &   1,6     &\nodata&                          \\     
 10&04 56 11.0   &-66 17 33.0 &BAT99 9;         Brey 7;    HD 32125            &14.33&WC4             &   1,6     & (10)  &                          \\     
 11&04 56 34.63  &-66 28 26.4 &BAT99 10;      Brey 9;    HD 32228              &10.83&WC4+OB          &   1,6     &    9  &  Crowded\tablenotemark{c}   \\          
 12&04 57 24.10  &-68 23 57.3 &BAT99 11;      Brey 10;  HD 32402               &12.96&WC4             &   1,6     &   12  & SW mem.\ pair             \\          
 13&04 56 48.79  &-69 36 40.7 &[MNM2015]LMCe055-1;  OGLE-LMC-ECL-3548          &16.15&WN4/O4          &   8       &\nodata&                    \\           
 14&04 57 27.44  &-67 39 02.9 &BAT99 12;      Sk$-67^\circ$22                  &13.50&O2If*/WN5       &   9       &\nodata&                    \\           
 15&04 57 41.04  &-66 32 42.6 &BAT99 13;      Sk$-66^\circ$40                  &12.85&WN10            &   10      & (9)  &                     \\          
 16&04 58 56.72  &-68 48 11.0 &BAT99 14;      Brey 11;        HD 268856        &10.83&WN4+OB          &   2,11    &\nodata&                    \\           
 17&04 59 51.55  &-67 56 55.4 &BAT99 15;        Brey 12;      HD 268847        &14.54&WN3             &   12      &\nodata&                      \\  
 18&05 02 59.24  &-69 14 02.3 &BAT99 15a;   [M2002]LMC 57799                   &15.33&WN3+abs         &   7       &\nodata& Candidate WN3/O3       \\       
 19&05 03 08.91  &-66 40 57.5 &BAT99 16;    Brey 13;          HD 33133         &12.70&WN7h            &   2,12    &\nodata& H em.\ present      \\          
 20&05 04 12.33  &-70 03 55.4 &BAT99 17;    Brey 14;          HD 269015        &14.17&WN4             &   1,2,3   &\nodata& WN3?               \\          
 21&05 04 32.64  &-68 00 59.4 &[MNM2014]LMC277-2                               &15.83&WN3/O3          &   13      &\nodata&                     \\          
 22&05 05 08.43  &-70 22 45.1 &BAT99 18;    Brey 15;          Sk$-70^\circ$64  &14.67&WN3h             &   14      & (18)  & H em.\ weakly present \\          
 23&05 07 13.33  &-70 33 33.9 &[MNM2014]LMC079-1;  [M2002]LMC 71747            &16.31&WN3/O3          &   13      &\nodata&                     \\          
 24&05 09 40.42  &-68 53 24.8 &BAT99 19;    Brey 16;          HD 34169         &13.75&WN3+OB          &   1       &   31  &  SB\tablenotemark{b}       \\          
 25&05 09 53.77  &-68 52 52.5 &BAT99 20;    Brey 16a;         [M2002]LMC 81268 &13.74&WC4             &   15      &   31  &                     \\          
 26&05 13 43.77  &-67 22 29.4 &BAT99 21;    Brey 17;          HD 34632         &13.16&WN4+OB          &   2,11    &   37  &                     \\          
 27&05 13 54.27  &-69 31 46.7 &BAT99 22;    Brey 18;          HD 269227        &12.04&WN9             &   10      &   39  &                     \\          
 28&05 13 56.01  &-67 24 36.6 &BAT99 23                                        &17.13&WN3             &   2,16    &   37  &                     \\          
 29&05 14 12.69  &-69 19 26.2 &BAT99 24;    Brey 19;          HD 34783         &14.29&WN3             &   1,2,11  & (35)  &                     \\          
 30&05 14 17.57  &-67 20 35.1 &[MNM2015]LMCe132-1                              &14.34&O3.5If*/WN5     &   17      & (36)  & SWrn of 3\farcs5 pair  \\       
 31&05 14 57.27  &-71 36 18.3 &BAT99 25;    Brey 19a                           &15.11&WN4ha           &   2,14    &\nodata&                    \\           
 32&05 16 38.84  &-69 16 40.9 &BAT99 26;    Brey 20;          Sk$-69^\circ$86  &14.60&WN4             &   1,2,3   & (41)  &                    \\           
 33&05 18 10.33  &-69 13 02.5 &[MNM2014]LMC195-1                               &15.15&WO4             &   13      &   41  & Crowded; FC in Ref.\ 13             \\          
 34&05 18 10.88  &-69 13 11.4 &[L72]LH41-1042                                  &14.00&WO4             &   18      &   41  & Crowded; FC in Ref.\ 13             \\          
 35&05 18 19.21  &-69 11 40.7 &BAT99 27;    Brey 21;          HD 269333        &11.21&BI+WN4          &   2       &   41  & B spectrum dominates  \\        
 36&05 19 16.34  &-69 39 20.0 &BAT99 28;    Brey 22; RMC 89\tablenotemark{d}   &12.21&WC6+O5-6        &   19      &   42  &                     \\          
 37&05 20 44.73  &-65 28 20.5 &BAT99 29;    Brey 23;          Sk$-65^\circ$45  &14.55&WN3+OB          &   1,2,3   &   43  &  SB\tablenotemark{b}                  \\           
 38&05 21 22.82  &-65 52 48.8 &[MNM2015]LMC169-1                               &17.12&WN3/O3          &   17      &\nodata&                     \\          
 39&05 21 57.70  &-65 49 00.3 &BAT99 30;    Brey 24;          Sk$-65^\circ$55  &13.30&WN6h            &   1,2,20  &\nodata& H em.\ strongly present \\      
 40&05 22 04.41  &-67 59 06.8 &BAT99 31;    Brey 25                            &15.21&WN3             &   1,2,3   &   47  &  SB?\tablenotemark{b}                      \\        
 41&05 22 22.53  &-71 35 58.1 &BAT99 32;    Brey 26;          HD 36063         &12.30&WN6h            &   1,2,21  &\nodata& H em.\ present       \\         
 42&05 22 59.78  &-68 01 46.6 &BAT99 33;    HD 269445                          &11.51&Ofpe/WN9        &   22      &   49  &                     \\          
 43&05 23 10.06  &-71 20 50.9 &BAT99 34;    Brey 28;          HD 36156         &12.66&WC4+abs         &   6       &\nodata&                     \\          
 44&05 23 18.01  &-65 56 57.0 &BAT99 35;    Brey 27                            &14.88&WN3             &   1,2,3   &\nodata& H em.\ weakly present  \\       
 45&05 24 24.19  &-68 31 35.6 &BAT99 36;    Brey 29                            &14.37&WN3/WCE+OB      &   1,2,3   &\nodata&                    \\           
 46&05 24 54.34  &-66 14 11.1 &BAT99 37;    Brey 30                            &16.33&WN3             &   2,14    & (52)  &                     \\          
 47&05 26 03.96  &-67 29 57.1 &BAT99 38;    Brey 31;          HD 36402         &11.62&WC4+abs         &   6       &   54  &                    \\           
 48&05 24 56.87  &-66 26 44.4 &[MNM2015]LMC159-1                               &16.34&WN3/O3          &   17      &\nodata& SErn of 3\farcs5 pair  \\        
 49&05 26 30.26  &-68 50 27.5 &BAT99 39;    Brey 32;          HD 36521         &12.32&WC4+O6III/V     &   1,19    &   58  &                     \\          
 50&05 26 36.86  &-68 51 01.3 &BAT99 40;    Brey 33                            &14.77&WN4             &   1,2,20  &   58  &                      \\         
 51&05 26 42.58  &-69 06 57.4 &BAT99 41;    Brey 35;          HD 269549        &14.71&WN4             &   1,2,3   &\nodata&                   \\            
 52&05 26 45.32  &-68 49 52.8 &BAT99 42;    Brey 34;          HD 269546        & 9.86&B3I+WN5         &   14      &   58  & B spectrum dominates     \\         
 53&05 27 37.68  &-70 36 05.4 &BAT99 43;    Brey 37;          Sk$-70^\circ$92  &14.08&WN3+OB          &   1,2,12  &\nodata& SB\tablenotemark{b}    \\          
 54&05 27 42.69  &-69 10 00.4 &BAT99 44;    Brey 36;          Sk$-69^\circ$141 &13.43&WN7h            &   1,2,23  &\nodata& H em.\ strongly  present \\     
 55&05 27 52.66  &-68 59 08.5 &BAT99 45;    HD 269582                          &12.60&WN10$\rightarrow$LBV            &   21,32     &\nodata&                      \\         
 56&05 28 17.90  &-69 02 35.9 &BAT99 46;    Brey 38                            &15.29&WN4             &   1,2,3   &\nodata&                     \\          
 57&05 28 27.12  &-69 06 36.2 &[MNM2014]LMC199-1                               &16.65&WN3/O3          &   13      &\nodata&                      \\         
 58&05 29 12.37  &-68 45 36.1 &BAT99 47;    Brey 39;          HD 269618        &15.30&WN3             &   2,11    &   64  &                      \\         
 59&05 29 18.19  &-69 19 43.2 &[MNM2014]LMC170-2;    [M2002]LMC 143741         &16.13&WN3/O3          &   13      &\nodata&                      \\         
 60&05 29 31.64  &-68 54 28.8 &BAT99 48;    Brey 40;          HD 269624        &14.78&WN3             &   1,2,11  & (64)  &                      \\         
 61&05 29 33.21  &-70 59 34.9 &BAT99 49;    Sk$-71^\circ$34                    &13.48&WN3+O7.5        &   2,24    & (66)  &  SB2\tablenotemark{b,e}  \\         
 62&05 29 53.64  &-69 01 04.8 &BAT99 50;    Brey 41                            &14.52&WN5h            &   2,25    &\nodata& NW mem.\ pair; H em.\ present       \\         
 63&05 30 02.46  &-68 45 18.4 &BAT99 51;    Brey 42                            &15.20&WN3             &   2,3     & (64)  &                    \\           
 64&05 30 12.16  &-67 26 08.3 &BAT99 52;    Brey 43                            &13.56&WC4             &   6       &  \nodata&                    \\           
 65&05 30 38.70  &-71 01 47.8 &BAT99 53;    Brey 44;          HD 37248         &12.96&WC4+abs         &   6       & (69)  &                    \\           
 66&05 31 18.05  &-69 08 45.5 &BAT99 54;    LMC AB 18                          &14.30&WN9             &   21      & (74)  &                     \\          
 67&05 31 25.52  &-69 05 38.6 &BAT99 55;    HD 269687                          &11.87&WN11            &   21      &\nodata&                     \\          
 68&05 31 32.87  &-67 40 46.6 &BAT99 56;    Brey 46;          HD 269692        &14.65&WN3             &   1,2,12  & (76)  & Runaway\tablenotemark{b}  \\          
 69&05 31 34.36  &-67 16 29.3 &BAT99 57;    Brey 45                            &14.90&WN3             &   1,2,3   & (70)  & Runaway\tablenotemark{b}    \\           
 70&05 32 07.49  &-68 26 31.6 &BAT99 58;    Brey 47                            &15.06&WN7h            &   1,2,26  &\nodata& H em.\ strongly present \\      
 71&05 33 10.57  &-67 42 43.1 &BAT99 59;    Brey 48;          HD 269748        &13.19&WN3+OB          &   2,12    & (76)  &   SB?\tablenotemark{b}      \\          
 72&05 33 10.87  &-69 29 01.0 &BAT99 60;    Brey 49                            &14.30&WN3+OB          &   1,2,11  &\nodata&                     \\          
 73&05 34 19.24  &-69 45 10.3 &BAT99 61;    Brey 50;          HD 37680         &13.12&WC4             &   1,6     &   81  &                    \\           
 74&05 34 36.08  &-69 45 36.5 &Sk$-69^\circ$194                                &11.91&B0I+WN          &   27      &   81  & B spectrum dominates  \\        
 75&05 34 37.47  &-66 14 38.0 &BAT99 62;    Brey 51                            &15.31&WN3             &   1,2,11  &\nodata&                      \\         
 76&05 34 52.03  &-67 21 29.0 &BAT99 63;    Brey 52                            &14.60&WN4h            &   1,2,20  & (79)  & H em.\ present. Runaway?\tablenotemark{f}       \\         
 77&05 34 59.38  &-69 44 06.3 &BAT99 64;    Brey 53                            &14.07&WN3+O           &   2       &   81  & SB\tablenotemark{b}  \\  
 78&05 35 00.90  &-69 21 20.2 &[MNM2014]LMC172-1                               &15.95&WN3/O3          &   13      &\nodata& E mem of pair                     \\          
 79&05 35 15.18  &-69 05 43.1 &BAT99 65;    Brey 55                            &15.39&WN3             &   2       & (89)  &  \\   
 80&05 35 28.52  &-69 40 08.9 &[NMN2014]LMC143-1                               &14.09&WN3+O8-9III     &   13      &   87  &                      \\         
 81&05 35 29.80  &-67 06 49.4 &BAT99 66;    Brey 54                            &15.36&WN3(h)          &   2,14    & (84)  &                     \\          
 82&05 35 41.96  &-69 11 52.9 &BAT99 69;    TSWR4                              &16.52&WC4             &   28      &   90  & Crowded\tablenotemark{c} \\                     
 83&05 35 42.19  &-69 12 34.5 &BAT99 67;    Brey 56                            &13.59&WN5h            &   1,2,14  &   90  & H em.\ present  \\              
 84&05 35 42.20  &-69 11 53.6 &BAT99 68;    Brey 58                            &13.59&O3.5If*/WN7     &   9       &   90  & Crowded\tablenotemark{c} \\
 85&05 35 43.49  &-69 10 58.0 &BAT99 70;    Brey 62                            &13.96&WC4             &   6       &   90  &                    \\           
 86&05 35 44.28  &-68 59 36.8 &BAT99 71;    Brey 60                            &14.78&WN3+abs         &   1,2     &   89  &  SB\tablenotemark{b}      \\           
 87&05 35 45.03  &-68 58 44.4 &BAT99 72;    Brey 61                            &15.38&WN4+abs         &   2,3     &   89  & SB?\tablenotemark{b} or candidate WN4/O4      \\        
 88&05 35 50.65  &-68 53 39.2 &BAT99 73;    Brey 63                            &14.64&WN5             &   2,25    &   85  &                      \\         
 89&05 35 52.43  &-68 55 08.7 &BAT99 74;    Brey 63a                           &15.58&WN3+abs         &   2,29    &   89  & Abs strong. WN3/O3 candidate             \\       
 90&05 35 54.03  &-67 02 48.9 &BAT99 75;    Brey 59                            &14.47&WN4             &   2,14    & (84)  &                      \\         
 91&05 35 54.37  &-68 59 07.9 &BAT99 76;    [BE74]381                          &13.27&WN9             &   10      &   89  &                      \\         
 92&05 35 58.87  &-69 11 47.8 &BAT99 77;    Brey 65                            &13.09&WN7             &   30      &   90  & Bright W component; FC in BAT99  \\          
 93&05 35 59.16  &-69 11 50.7 &BAT99 78;    Brey 65b                           &14.59&WN4             &   30      &   90  & Crowded\tablenotemark{c}. HM-5C in Ref.\ 30 \\            
 94&05 35 59.82  &-69 11 22.3 &BAT99 79;    Brey 57                            &13.49&WN7             &   1,2,23  &   90  &                     \\          
 95&05 35 59.89  &-69 11 50.6 &BAT99 80;    TSWR2,N2044W-9A                    &13.02&WN5\tablenotemark{g}        &   2,23,30 &   90  & Crowded\tablenotemark{c}; O4~If$^+$?\tablenotemark{g}  \\                            
 96&05 36 12.13  &-67 34 57.8 &BAT99 81;    Brey 65a                           &15.39&WN5h            &   2,31    &   88  & H em.\ strongly present; Runaway?\tablenotemark{f} WN6h?     \\  
 97&05 36 33.58  &-69 09 17.3 &BAT99 82;    Brey 66                            &16.11&WN3             &   3       &   90  &                     \\          
 98&05 36 43.71  &-69 29 47.5 &BAT99 83;    R127;  HD 269858;                  & 9.30&Ofpe/WN9$\rightarrow$LBV   &   22,32   &   94  &Currently in S Dor state\\         
 99&05 36 51.38  &-69 25 56.7 &BAT99 84;    Brey 68;          HD 38030         &12.99&WC4(+OB)        &   15      &   93  &                      \\         
100&05 36 54.66  &-69 11 38.3 &BAT99 85;    Brey 67                            &12.18&WC4(+OB)        &   15      &   (90)  &                         \\      
101&05 37 11.48  &-69 07 38.2 &BAT99 86;    Brey 69                            &16.30&WN3             &   2,33    & (100)  & \\                              
102&05 37 29.24  &-69 20 47.5 &BAT99 87;    Brey 70                            &13.69&WC4             &   2,6     &   97  & "Close to WO;" see Ref.\ 15\\   
103&05 37 35.72  &-69 08 40.3 &BAT99 88;    Brey 70a                           &16.92&WN3/WCE         &   2       &   99  & CIV 5806 $>$ He\,{\sc ii}; N\,{\sc iv}$<<$ N\,{\sc v} \\  
104&05 37 40.50  &-69 07 57.7 &BAT99 89;    Brey 71                            &14.08&WN6             &   2       &   99  & N\,{\sc v} weak but present  \\         
105&05 37 44.64  &-69 14 25.7 &BAT99 90;    Brey 74;          HD 269888        &14.63&WC4             &   2,15    & (99)  &                     \\          
106&05 37 46.35  &-69 09 09.6 &BAT99 91;    Brey 73                            &14.75&WN6h            &   2,30,33 &   99  & Crowded.\tablenotemark{c} H em.\ strongly present\\       
107&05 37 47.62  &-69 21 13.6 &[NMN2014]LMC173-1;    [M2002]LMC 169271         &14.65&WN3+O7V         &   13      &   97  &                     \\          
108&05 37 49.04  &-69 05 08.3 &BAT99 92;    Brey 72;          HD 269891        &11.62&B1I+WN3         &   23      &  100  & B spectrum dominates   \\       
109&05 37 51.34  &-69 09 46.7 &BAT99 93;    LH99-3                             &13.45&O3If*           &   9       &   99  & Downgraded from O3If/WN6 \\     
110&05 38 24.21  &-69 29 13.4 &[NMN2015]LMCe063-1; Sk$-69^\circ$240            &13.04&WN11            &   17      & (101)  &                      \\         
111&05 38 27.71  &-69 29 58.5 &BAT99 94;    Brey 85;          HD 269908        &14.71&WN3/4pec        &   1,2,3   &  101  & Lines unusually broad\\         
112&05 38 33.62  &-69 04 50.5 &BAT99 95;    Brey 80;          HD 269919        &13.50&WN7             &   2,12    &  100  &                   \\            
113&05 38 36.42  &-69 06 57.4 &BAT99 96;    Brey 81                            &13.74&WN7             &   2       &  100  &  \\
114&05 38 38.84  &-69 06 49.5 &BAT99 97;   [P93]666                            &13.73&O3.5If*/WN7     &   33      &  100  &                      \\         
115&05 38 39.15  &-69 06 21.2 &BAT99 98;    Brey 79                            &13.67&WN6             &   23      &  100  &           \\                    
116&05 38 40.228 &-69 05 59.81&R136-007;    Mk39;            BAT99 99          &13.01&O2.5If*/WN6     &   9,34    &  100  &  Crowded\tablenotemark{h}  \\                          
117&05 38 40.551 &-69 05 57.14&R136-004;    R134; BAT99 100                    &12.89&WN6h            &   34      &  100  & Crowded\tablenotemark{h}   \\                   
118&05 38 41.60  &-69 05 14.0 &BAT99 101;   R140a1                             &12.20&WC4             &   15,35   &  100  & Crowded\tablenotemark{h}                     \\         
119&05 38 41.60  &-69 05 14.0 &BAT99 102;   R140a2                             &12.20&WN6             &   23      &  100  & Crowded\tablenotemark{c}   \\         
120&05 38 41.62  &-69 05 15.1 &BAT99 103;   R140b                              &12.80&WN5(h)+O        &   33      &  100  & Crowded\tablenotemark{c}    \\           
121&05 38 41.875 &-69 06 14.39&R136-044;    BAT99 104                          &14.66&O2If*/WN5       &   9,34    &  100  & Crowded\tablenotemark{h}   \\                          
122&05 38 42.116 &-69 05 55.22&R136-002;    BAT99 105;       Mk42              &12.84&O2If*  &   34,9   &  100  & Crowded.\tablenotemark{h}Downgraded from O3If*/WN6   \\                          
123&05 38 42.333 &-69 06 03.30&R136-006;    R136a3;          BAT99 106         &13.01&WN4.5h          &   34      &  100  & Crowded\tablenotemark{h}                    \\          
124&05 38 42.390 &-69 06 02.95&R136a1;      BAT99 108                          &12.84&WN5h            &   36      &  100  & Crowded\tablenotemark{h}  \\          
125&05 38 42.408 &-69 06 15.04&R136-015;    Mk30                               &13.59&O2If*/WN5       &   9,34   &  100  &   \\                            
126&05 38 42.412 &-69 06 02.89&R136a2;      BAT99 109                          &12.96&WN5h            &   36      &  100  & Crowded\tablenotemark{c}   \\          
127&05 38 42.430 &-69 06 02.75&R136-020;    R136a5;          BAT99 110         &13.93&O2If*/O3If*/WN6 &   9,34    &  100  &  Crowded\tablenotemark{h} \\                           
128&05 38 42.906 &-69 06 04.85&R136-010;    BAT99 112                          &13.47&WN4.5h          &   34      &  100  &  Crowded\tablenotemark{h}  \\          
129&05 38 43.10  &-69 05 46.8 &R136-015;    BAT99 113                          &13.30&O2If*/WN5       &   9       &  100  & Crowded\tablenotemark{h} \\          
130&05 38 43.211 &-69 06 14.40&R136-012;    Mk35;            BAT99 114         &13.54&O2If*/WN5       &   9,34    &  100  & Crowded\tablenotemark{h} \\                           
131&05 38 44.063 &-69 05 55.57&R136-034;    BAT99 115                          &14.47&WC5             &   34      &  100  &  Crowded\tablenotemark{h}            \\                
132&05 38 44.257 &-69 06 05.88&R136-008;    Mk34;            BAT99 116         &13.30&WN4.5h          &   34      &  100  &  Crowded\tablenotemark{h}  \\               
133&05 38 47.52  &-69 00 25.3 &BAT99 117;   Brey 88;          HD 269926        &13.12&WN4.5           &   2       &  100  &  N\,{\sc iv}$>$N\,{\sc v}$>>$N\,{\sc iii}; Runaway\tablenotemark{b}     \\            
134&05 38 53.38  &-69 02 00.9 &BAT99 118;   R144                               &11.11&WN5/6+WN6/7\tablenotemark{i} &   37      &  100  &  WN6h composite type    \\     
135&05 38 55.53  &-69 04 26.7 &[P93]1732;   VFTS682                            &16.08&WN5h            &   38      &\nodata&                     \\          
136&05 38 57.07  &-69 06 05.7 &BAT99 119;   Brey 90;          R145             &11.94&WN6+O3.5If*/WN7 &   39      &  100  &                   \\            
137&05 38 58.09  &-69 29 19.5 &BAT99 120;   Brey 91;          5-68             &12.63&WN9             &   40      &  101  &  \\    
138&05 39 03.78  &-69 03 46.5 &BAT99 121;   [P93]1974                          &15.83&WC4             &   15      &  100  &                     \\          
139&05 39 11.33  &-69 02 01.6 &BAT99 122;   Brey 92;          HD 38344         &13.07&WN5h            &   2,14    &  100  &                     \\          
140&05 39 34.29  &-68 44 09.2 &BAT99 123;   Sand 2;          Brey 93           &15.20&WO3             &   41      &\nodata&                     \\          
141&05 39 36.18  &-69 39 11.2 &BAT99 124;   Brey 93a                           &14.86&WN3             &   2,42    &  103  & NE component; strong neb.            \\       
142&05 39 56.11  &-69 24 24.3 &BAT99 125;   Brey 94;          HD 38448         &13.00&WC4+abs         &   6       &  104  &                     \\          
143&05 40 03.57  &-69 37 53.1 &[MNM2014]LMC174-1                               &17.02&WN3/O3          &   13      &  103  & NW mem.\ of pair                      \\         
144&05 40 07.55  &-69 24 31.9 &BAT99 126;   HD 38472;         Brey 95          &13.17&WN3+O7          &   2,40    &  104  &  SB?\tablenotemark{b,j}     \\           
145&05 40 13.06  &-69 24 04.2 &BAT99 127;   [ST92]4-102                        &13.30&WC4+O           &   15      &  104  &  W mem.\ of pair                   \\          
146&05 40 13.33  &-69 22 46.5 &[MNM2014]LMC174-5;    HD 38489                  &12.22&B[e]+WN?        &   13      &  104  & Broad He\,{\sc ii} $\lambda4686$ em.\\     
147&05 40 50.80  &-69 26 31.8 &BAT99 128;   Brey 96                            &15.02&WN3             &   2,11    & (104)  & Runaway?\tablenotemark{b}       \\       
148&05 41 17.50  &-69 06 56.2 &[MNM2015]LMCe078-3                              &17.03&WN3/O3          &   8       & (111)  &                        \\
149&05 41 48.57  &-70 35 30.8 &BAT99 129;   Brey 97                            &14.70&WN3+O5V         &   43      &\nodata& SB\tablenotemark{b}              \\         
150&05 44 31.03  &-69 20 15.5 &BAT99 130;   Sk$-69^\circ$296                   &12.72&WN11            &   21      &\nodata&                     \\          
151&05 44 53.72  &-67 10 36.2 &BAT99 131;   Brey 98;  Sk$-67^\circ$259         &14.36&WN4             &   2,14    &  116  &                     \\          
152&05 45 24.16  &-67 05 56.8 &BAT99 132;   Brey 99                            &14.62&WN4             &   2,14    & (116)  & Runaway?\tablenotemark{b}                     \\         
153&05 45 51.93  &-67 14 25.9 &BAT99 133;   Sk$-67^\circ$266                   &12.10&WN11            &   21      &  116  &           \\     
154&05 46 46.35  &-67 09 58.3 &BAT99 134;   HD 270149                          &14.50&WN3             &   2       & (116)  & \\
\enddata                                                                                                                                              
\tablecomments{The following stars were included in BAT99 as WRs, but are not included here as they've been reclassified as O-type stars: 
BAT99 6 (now O3f$^*$+O binary,\citealt{2001A&A...369..544N}),  BAT99 107 (now O6.5Iafc+O6Iaf, \citealt{2014A&A...564A..40W}).}
\tablerefs{                                                                                                                                           
(1) Spectrum re-examined here using old SIT-Vidicon spectra described in \citealt{1983ApJ...264..126M} and \citealt{1987ApJS...65..459T};             
(2)  Spectrum re-examined here based upon the spectra shown in \citealt{2014yCat..35650027H};                                                                     
(3)  \citealt{1983ApJ...264..126M};                                                                                                                   
(4)  \citealt{2014MNRAS.442..929G};                                                                                                                   
(5)  \citealt{1991A&A...244L...9M};                                                                                                                   
(6)  \citealt{1986ApJ...300..379T};                                                                                                                   
(7)  \citealt{2012MNRAS.426.1867H};                                                                                                                   
(8)  \citealt{PaperIII};                                                                                                                   
(9)  \citealt{2011MNRAS.416.1311C};                                                                                                                   
(10) \citealt{1995A&A...293..172C};                                                                                                                   
(11) \citealt{1981A&AS...43..203B};                                                                                                                   
(12) \citealt{1983ApJ...268..228C};                                                                                                                   
(13) \citealt{PaperI};                                                                                                                          
(14) \citealt{2003MNRAS.338.1025F};                                                                                                                   
(15) \citealt{2001MNRAS.324...18B};                                                                                                                   
(16) \citealt{1999MNRAS.305..469M};                                                                                                                   
(17) \citealt{PaperII};                                                                                                                          
(18) \citealt{NeugentWO};                                                                                                                   
(19) \citealt{1990ApJ...348..232M};                                                                                                                   
(20) \citealt{1996MNRAS.281..163S};                                                                                                                   
(21) \citealt{1997A&A...320..500C};                                                                                                                   
(22) \citealt{1989PASP..101..520B}                                                                                                                    
(23) \citealt{2008MNRAS.389..806S};                                                                                                                   
(24) \citealt{1995ApJ...438..188M};                                                                                                                   
(25) \citealt{2006A&A...449..711C};                                                                                                                   
(26) \citealt{1992A&AS...93..495M};                                                                                                                   
(27) \citealt{Waterhouse};                                                                                                                            
(28) \citealt{1993A&A...280..426T};                                                                                                                   
(29) \citealt{1985MNRAS.216..459M};                                                                                                                   
(30) \citealt{1999AJ....118.1684W};                                                                                                                   
(31) \citealt{1984PASP...96..968C};                                                                                                                   
(32) \citealt{2017AJ....154...15W};                                                                                                                   
(33) \citealt{2011A&A...530A.108E};                                                                                                                   
(34) \citealt{MH98};                                                                                                                                  
(35) \citealt{1987ApJ...312..612M};                                                                                                                   
(36) \citealt{2010MNRAS.408..731C};                                                                                                                   
(37) \citealt{2013MNRAS.432L..26S};                                                                                                                   
(38) \citealt{2012A&A...542A..49B};                                                                                                                   
(39) \citealt{2017A&A...598A..85S};                                                                                                                   
(40) \citealt{1998A&AS..130..527T};                                                                                                                   
(41) \citealt{1998MNRAS.296..367C};                                                                                                                   
(42) \citealt{1986A&A...162..180H};                                                                                                                   
(43) \citealt{2006A&A...447..667F};                                                                                                                    
}                                                                                                                                                                                                                                                                                                         
\tablenotetext{a}{\phantom{}Lucke-Hodge (LH) OB association numbers are from \citealt{LuckeHodge} and \citealt{LuckePhD}.  Parenthesis are used to denote the association if the star is only near the association.  Note that the 30~Dor region corresponds to LH~100 and its extension to the SW LH~99, while the center of Constellation~III is LH~84.
}                                                                                                                                                     
\tablenotetext{b}{From \citealt{2003MNRAS.338.1025F}.}  
\tablenotetext{c}{Crowded; see finding chart in BAT99.}
\tablenotetext{d}{Note that this star is not HD~35517, but rather its south-preceeding companion, RMC 89.  See \citealt{1987BICDS..33..119B}.}
\tablenotetext{e}{From \citealt{1991IAUS..143..201N}.}
\tablenotetext{f}{From \citealt{1984PASP...96..968C}.}
\tablenotetext{g}{We have retained the WN5 classification of BAT99 80 despite the reclassification by \citealt{1999AJ....118.1684W} as a O4~If+ based upon
an {\it HST} Faint Object Spectrogaph (FOS) spectrum.  Although \citealt{1999AJ....118.1684W}  were able to separate this star ("5C") in the tight cluster that contains Brey 65 and numerous
other early-type stars, there are some problems.  The ground-based spectrum modeled by \citealt{PotsLMC}  shows N\,{\sc iii}, N\,{\sc iv}, and N\,{\sc v} 
emission of roughly comparable strength, as well as He\,{\sc ii} $\lambda$5411 emission.  If this is simply due to contamination by Brey 65, though, where is the N\,{\sc v} emission coming from?  Brey 65 is a WN7 star, and its spectrum has strong N\,{\sc iii}, weak N\,{\sc iv} and no N\,{\sc v}.  So, it is hard to see how the problem is simply contamination. The {\it HST} FOS spectrum is of low S/N and if N\,{\sc iv} and N\,{\sc v}  were present as shown in the ground-based spectrum, we doubt that it would appear.  A new spectrum taken under excellent seeing conditions would be useful in resolving this.}
\tablenotetext{h}{Crowded; see finding charts in BAT99 and \citealt{MH98}.}
\tablenotetext{i}{Described as an SB2 by \citealt{2013MNRAS.432L..26S} but fit with a single set of parameters by \citealt{PotsLMC}.}
\tablenotetext{j}{From \citealt{1998A&AS..130..527T}.}
\end{deluxetable}                                                                                                                                     

